On the Regret of Coded Caching with Adversarial Requests

We study the well-known coded caching problem in an online learning framework, wherein requests arrive sequentially, and an online policy can update the cache contents based on the history of requests seen thus far. We introduce a caching policy based on the Follow-The-Perturbed-Leader principle and show that for any time horizon T and any request sequence, it achieves a sub-linear regret of \mathcal{O}(\sqrt(T) ) with respect to an oracle that knows the request sequence beforehand. Our study marks the first examination of adversarial regret in the coded caching setup. Furthermore, we also address the issue of switching cost by establishing an upper bound on the expected number of cache updates made by our algorithm under unrestricted switching and also provide an upper bound on the regret under restricted switching when cache updates can only happen in a pre-specified subset of timeslots. Finally, we validate our theoretical insights with numerical results using a real-world dataset

==> Ourpolicy1a.tex <==
%\section{Our Online Subset selection Algorithm}
%\section{Our Online Subset selection Algorithm}

\section{Our Algorithm}
\label{section: policy}
\begin{algorithm}[tb]
\SetAlgoLined
\footnotesize
\caption{Algorithm for Adversarial Coded Caching}\label{alg:FTPL}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $M, N, T, \mathbf{s}_0=[1,1\cdots 1], \mathcal{T}, (\eta_t)_{t\in \mathcal{T}} $
\STATE Sample $\gamma \sim \mathcal{N}(0,\textit{I}_{N\times N}) $
\FOR{$t \leq T$}
   \STATE \textbf{Placement phase}:
   %\STATE \textbf{Subset selection for placement}:
   \STATE $\mathbf{y}_{t-1} \gets \min\{\mathbf{x}_{t-1}, \mathbb{I}_N\} $
   \STATE $\mathbf{Y}_{t} \gets \mathbf{Y}_{t-1} + \mathbf{y}_{t-1}$
   \IF {$t\in \mathcal{T}$}
      \STATE $\overline{\mathbf{Y}}_{t} = \mathbf{Y}_{t} - \eta_{t}\gamma$
      \STATE \textbf{Subset selection for placement}:
      \STATE $\mathbf{s}_{t} \gets \arg \min_{\mathbf{s}\in\mathcal{S}} \left\langle\left(\mathbf{s} - \frac{M}{N}\mathbb{I}_N\right), \sum_{i = 1}^{t-1}f(\mathbf{x}_i,s) -\overline{\mathbf{Y}}_{t} \right\rangle $
      \STATE Perform cache placement with $\mathbf{s}_t$ according to the placement phase of Section \ref{sec:sysmodel}
   \ENDIF
   \STATE \textbf{Delivery phase}:
   \STATE Receive $\mathbf{x}_{t}$
   \STATE Perform content delivery according to the delivery phase of Section \ref{sec:sysmodel}
\ENDFOR
\end{algorithmic}
\end{algorithm}


In this section, we present our online algorithm, which achieves $\mathcal{O}(\sqrt{T})$ regret. Our algorithm is a variant of the standard FTPL algorithm commonly used in online learning settings, and its pseudocode is provided in Algorithm \ref{alg:FTPL}. Our algorithm aims to identify a subset of files, $\mathbf{s}_t$, to be cached in each time slot $t \in \mathcal{T}$, guided by the history of request patterns.

In the single-user caching setting, FTPL is similar to LFU, which monitors the frequency of each file's requests. However, it distinguishes itself by selecting the top $M$ files after introducing a Gaussian perturbation to the cumulative request numbers. The FTPL policy has been extensively studied (see \cite{mukhopadhyay2021online,bhattacharjee2020fundamental,paria2021texttt}) and demonstrated to achieve $\mathcal{O}(\sqrt{T})$ regret in adversarial settings. The rate expression in this setting is linear in both policy parameters $\mathbf{s}_t$ and past observations, as a result of which the choice of cache configuration is simply the set of $M$ files with the maximum cumulative requests after perturbation. Since the expected rate expression in the coded caching setting is a non-linear function of the requests (of both request profile $\mathbf{r}_t$ and request pattern $\mathbf{x}_t$) as well as the cache configuration $(\mathbf{s}_t)$, introducing noise to requests makes the regret analysis challenging.

Now, we give a formal description of our algorithm. As we mentioned earlier, time is divided 

Nevertheless, it is noteworthy that the expected cumulative rate that would be incurred for any cache configuration $s$ until time $t$ given by $\sum_{i = 1}^{t-1} K(\mathbf{s},\mathbf{x}_i) = \left\langle\left(\mathbf{s}-\frac{M}{N}\mathbb{I}_N\right), \sum_{i = 1}^{t-1}f(\mathbf{s}_i,\mathbf{x})-\mathbf{\mathbf{Y}}_t\right\rangle +  \sum_{i = 1}^{t-1}h(\mathbf{x}_i),$ is linear in $\mathbf{Y}_t$. Here $\mathbf{Y}_t = \sum_{i=1}^{t-1}\mathbf{y}_i$ is a function of the requests. Our Algorithm relies on perturbing $\mathbf{Y}_t$ for subset selection at $t\in\mathcal{T}$. We demonstrate that it will yield similar performance guarantees to those achieved by FTPL in a single-user uncoded caching setting\footnote{The regret in the uncoded caching setting is calculated with respect to a static oracle, which chooses from only a class of uncoded policies and has inferior performance compared to the oracle here}. The perturbation used at time $T$ is $\eta_t \cdot \mathcal{N}(0,\textit{I}_{N\times N})$-independent Gaussian with zero mean and standard deviation $\eta_t$ in each dimension, where $\eta_t = \alpha\sqrt{t}$. 

The vector $\mathbf{y}_t$ is calculated, and $\mathbf{Y}_t$ is updated as detailed in lines 6-7 of Algorithm \ref{alg:FTPL}. The cumulative rate that would have been incurred by the cache configuration $\mathbf{s}$ until $t$ is given by $\left\langle\left(\mathbf{s} - \frac{M}{N}\mathbb{I}_N\right), \sum_{i = 1}^{t-1}f(\mathbf{x}_i,\mathbf{s})-\mathbf{Y}_t \right\rangle + \sum_{i=1}^{t-1}h(\mathbf{x}_i)$. For $t \in \mathcal{T}$, when we are allowed to change the cache configuration, the subset $\mathbf{s}_{t}$ of the files to be cached is then determined as the one that minimizes the cumulative rate until $t$ with the perturbed vector  $\overline{\mathbf{Y}}_t$ as shown in lines 8-11. The $h(\mathbf{x}_t)$ terms in the cumulative rate expression are ignored in this minimization as they do not depend on the policy parameters $\mathbf{s}$. After the subset selection, cache placement occurs according to the guidelines outlined in Section \ref{sec:sysmodel}. Subsequently, the delivery phase commences upon receiving requests, as depicted in lines 13 through 15.



==> results1a.tex <==
\section{Main Results}
\label{sec: Mainresults}
\begin{comment}
\subsection{Results for Stochastic setting}
Our first result outlines the regret incurred by the policy described in Algorithm \ref{alg:FTPL} w.r.t the stochastic oracle defined in equation (\ref{eq:r_stoc}). 
\begin{theorem}
    Let $\Delta_s = K(s) - K_o^S$. The regret incurred by the proposed online policy (Algorithm \ref{alg:FTPL}) and the placement delivery mechanism described above with a learning rate $\eta_t = \alpha\sqrt{t}$  is upper-bounded by 
    \begin{equation}
    R_{\eta}^S(T) \leq \sum_{s\in \mathcal{S}\setminus s^*} \frac{64}{\Delta_s}\left((r_{\max}^C)^2+K^2 +\frac{M^2\alpha^2}{N^2}\right)
\end{equation}
Here $r_{\max}^C$ is the maximum possible length of a coded transmission over the set of all possible requests $x_t$ and cache configurations $s_t$, and   $s^* = \arg\min_{s\in \mathcal{S}}K(s)$ is the cache configuration used by the oracle.
\end{theorem}
\begin{proof}
The proof for this theorem is available in Appendix \ref{app: stocub}. It relies on the idea that, given the users have a stationary preference distribution, the policy can learn the distribution of $f(x_t,s)$ for all $s$ and $y_t$ over time after observing an adequate number of request samples. Consequently, it deviates from the Oracle policy with low probability, which is described formally via the lemma \ref{lemma: probub}.
\end{proof}
Let $K_t^{\eta_t}(s) = \left\langle\left(s-\frac{M}{N}\mathbb{I}\right), \sum_{i=1}^t f(x_i,s)-Y_{t+1} +\eta_t \gamma \right\rangle $. Also, let $\mathcal{B}^t(s)$ be the event that $K_t^{\eta_t}(s)\leq K_t^{\eta_t}(s^*)$ (an event which will result in a choice of a wrong cache configuration). Note that the event that the policy chooses a cache configuration different from the oracle at time $t$ is a subset of the event $\bigcup_{s\in\mathcal{S}\setminus s^*}\mathcal{B}^t(s)$. Then we have
\begin{lemma}
The probability of the event $\mathcal{B}^t(s)$ is upper bounded by
    \begin{equation}
    \mathbb{P}(\mathcal{B}^t(s)) \leq  2\left(e^{-\frac{t\Delta_s^2}{32(r_{\max}^C)^2}}
      +  e^{-\frac{t\Delta_s^2} {32(K)^2}}+
      e^{-\frac{t\Delta_s^2N^2}{32M^2\alpha^2}}\right)
\end{equation}
\label{lemma: probub}
\end{lemma}
\begin{proof}
   The proof of the lemma is available in Appendix \ref{app: stoclemma} 
\end{proof}


The regret incurred in the stochastic case is thus upper-bounded by a constant, consistent with the results obtained in most online learning settings.
\begin{remark}
    Using lemma \ref{lemma: probub}, one can upper bound the performance under restricted switching and the number of times the cache configuration switches by constants for the stochastic case.
\end{remark}
The details are presented in Appendix \ref{app: stocswitch} and \ref{app: resstoc} due to the lack of space. 
\end{comment}
%\subsection{Results for Adversarial setting}
Now, we discuss the performance of our algorithm under the adversarial request setting. We evaluate the performance of our algorithm in two different scenarios. The first scenario is the unrestricted switching setting, with no restrictions on time slots wherein cache configurations can be switched; i.e., $\mathcal{T} = \{1,2\cdots T\}$, we are allowed to switch in every time slot. The second scenario is restricted switching, where we are allowed to switch only in a set of pre-specified time slots.
 

\subsubsection{Unrestricted Switching} 
Let $r_{\max}$ and $r_{\max}^C$ be the maximum length of the server transmission (coded + uncoded) and the maximum length of a coded transmission over all request pattern and cache configuration pairs, respectively. $|\mathcal{S}|$ is the cardinality of the set of feasible cache configurations. The following Theorem gives an upper bound on the adversarial regret of Algorithm \ref{alg:FTPL} with no restrictions on switching.
%Let $R_{(\eta, \text{UR})}^{A}(T)$ be the regret incurred by the policy (algorithm \ref{alg:FTPL}) with a learning schedule $\eta$ in the adversarial unrestricted switching case where cache configuration is allowed to change in every time slot.
\remove{\begin{theorem} \label{theorem:regret_unrestricted}
    The regret incurred by the proposed online policy (Algorithm \ref{alg:FTPL}) in the adversarial setting w.r.t. the oracle performance described in \eqref{eqn:oracle_performace_general} for a horizon $T$ can be upper bounded by
\begin{multline}
        R_{(\eta, \text{UR})}^{A}(T) \leq   r_{\max}^C  +\eta_T\mathcal{G}_{\max}(\gamma)+
         \\ \left(\frac{K^2}{\sqrt{2\pi}} +\frac{3r_{\max}r_{\max}^C|\mathcal{S}|}{2\sqrt{\pi}}\right)\sum_{t=1}^T\frac{1}{\eta_t} = \mathcal{O}(\sqrt{T}) 
\end{multline}
where \\
$\eta_t = \alpha\sqrt{t}$ and $\mathcal{G}_{\max}(\gamma)$ is the maximum Gaussian width given by
\begin{equation}
    \max_{a \in\mathcal{A}}\mathbb{E}_{\gamma}[\langle a,\gamma\rangle] 
\end{equation}
Here 
\[\mathcal{A} = \left\{a=[a_1,a_2,...,a_N]^T|a_i \in \{0,1\};\langle a, \mathbb{I}_N\rangle\geq M\right\} \]
and $\gamma \sim \mathcal{N}(0,\textit{I}_{N\times N})$.
This can be upper bounded as $\max_{M\leq  m\leq N}m\sqrt{\log(\frac{N}{m})}.$
\end{theorem}

\begin{theorem} \label{theorem:regret_unrestricted}
For an adversarial coded caching problem with $N$ files, $K$ users/caches and cache size $MF$ bits, let $ R_{(\eta, \text{UR})}(T)$  be the Algorithm \ref{alg:FTPL}'s adversarial regret with unrestricted switching and input parameters $\mathbf{\eta}=(\eta_t=\alpha\sqrt{t})_{t\in \mathcal{T}}$. Then, 
\begin{align*}
        R_{(\mathbf{\eta}, \text{UR})}^{A}(T) &\leq   r_{\max}^C  +\eta_T\mathcal{G}_{\max}(\gamma)+
         \\ &\left(\frac{K^2}{\sqrt{2\pi}} +\frac{3r_{\max}r_{\max}^C|\mathcal{S}|}{2\sqrt{\pi}}\right)\sum_{t=1}^T\frac{1}{\eta_t} = \mathcal{O}(\sqrt{T}) 
\end{align*}
where $\mathcal{G}_{\max}(\gamma)$ is the maximum Gaussian width given by
    $\max_{a \in\mathcal{A}}\mathbb{E}_{\gamma}[\langle a,\gamma\rangle]$ 
with
\[\mathcal{A} = \left\{a=[a_1,a_2,...,a_N]^T|a_i \in \{0,1\};\langle a, \mathbb{I}_N\rangle\geq M\right\} \]
and $\gamma \sim \mathcal{N}(0,\textit{I}_{N\times N})$.
$\mathcal{G}_{\max}(\gamma)$ can be upper bounded as $\max_{M\leq  m\leq N}m\sqrt{\log(\frac{N}{m})}.$
\end{theorem}}

\begin{theorem} \label{theorem:regret_unrestricted}
For an adversarial coded caching problem with $N$ files, $K$ users/caches, and cache size $MF$ bits, let $R_{(\eta, \text{UR})}(T)$ be the adversarial regret of Algorithm \ref{alg:FTPL} with unrestricted switching and input parameters $\mathbf{\eta}=(\eta_t=\alpha\sqrt{t})_{t\in \mathcal{T}}$. Then, 
\begin{align*}
    R_{(\mathbf{\eta}, \text{UR})}(T) &\leq r_{\max}^C + \eta_T \mathcal{G}_{\max}(\gamma) \\
    &+ \left(\frac{K^2}{\sqrt{2\pi}} + \frac{3r_{\max} r_{\max}^C |\mathcal{S}|}{2\sqrt{\pi}}\right) \sum_{t=1}^T \frac{1}{\eta_t} = \mathcal{O}(\sqrt{T}) 
\end{align*}
where $\mathcal{G}_{\max}(\gamma)$ is the maximum Gaussian width given by
$\max_{a \in \mathcal{A}} \mathbb{E}_{\gamma}[\langle a,\gamma\rangle]$ with
\[
\mathcal{A} = \left\{ a=[a_1,a_2,\ldots,a_N]^T \mid a_i \in \{0,1\}, \langle a, \mathbb{I}_N \rangle \geq M \right\}
\]
and $\gamma \sim \mathcal{N}(0,\textit{I}_{N\times N})$. $\mathcal{G}_{\max}(\gamma)$ can be upper bounded as $\max_{M\leq m \leq N} m\sqrt{\log(\frac{N}{m})}$.
\end{theorem}
%\begin{proof}
 %   A proof of the theorem is provided in Appendix \ref{app: advregret}
%\end{proof}
\begin{remark}
    Note that unlike the single-cache settings \cite{mukhopadhyay2021online,bhattacharjee2020fundamental,paria2021texttt}, the expected rate expression in the coded caching setting is a non-linear function of the requests (both request profile $r_t$ and request pattern $x_t$) as well as the cache configuration $s_t$ (See Proposition \ref{proposition:expected_rate}). However, similar to single-cache settings, Algorithm \ref{alg:FTPL} achieves $\mathcal{O}(\sqrt{T})$ regret for the coded caching problem.
\end{remark}


\remove{\begin{proof}
    {\color{red}A tighter expression for the upper bound and the complete proof of the theorem is provided in Appendix \ref{app: advregret}. Notably, a segment of the proof that helps us bound the non-linear $f(x,s)$ terms in the rate expression relies on the expected number of cache configuration switches performed by the policy until time $T$ being of the order $\mathcal{O}(\sqrt{T})$. This dependence was not necessary to provide an upper bound in the single-user uncoded caching setting. 
Note that since for a learning rate of $\alpha\sqrt{T}$ one can show that the term $\sum_{t=1}^T\frac{1}{\eta_t}\leq \frac{2}{\alpha}\sqrt{T}$ and minimize the upper bound expression w.r.t $\alpha$ to obtain the best value of alpha. Note that the values of $r_{\max}^C$ and $r_{\max}$ can be upper bounded by $K$, an upper bound of the maximum possible rate.} 
\end{proof}}
%\subsubsection{Switching cost}
As we mentioned in Section \ref{sec:sysmodel}, an algorithm that fetches a large number of files into the caches each time to change the cache configuration is not ideal as fetching files into the caches causes latency and consumes bandwidth.  Hence, in Theorem \ref{theorem:advswitch}, we upper bound the expected number of switches incurred by Algorithm \ref{alg:FTPL} under unrestricted switching.
% For our proposed algorithm, we now provide an upper bound on the expected switching cost in terms of the overall expected number of time slots until $T$, where the cache configuration $s$ gets updated. We show that the switching cost is of the same order as the regret incurred by the algorithm.
\begin{theorem}
\label{theorem:advswitch}
For an adversarial coded caching problem with $N$ files, $K$ users/caches, and cache size $MF$ bits, let $C_{(\mathbf{\eta}, \text{UR}) }(T)$ denote
the expected number of switches in cache configuration until time $T$ for Algorithm \ref{alg:FTPL} with unrestricted switching and input parameters $\mathbf{\eta}=(\eta_t=\alpha\sqrt{t})_{t\in \mathcal{T}}$. Then
\begin{equation}
   C_{(\mathbf{\eta}, \text{UR}) }(T) \leq \frac{3r_{\max}(|\mathcal{S}|-1)}{2\sqrt{\pi}} \sum_{t=2}^T \frac{1}{\eta_t} = \mathcal{O}(\sqrt{T}) \nonumber 
\end{equation}
where $|\mathcal{S}|$ is the cardinality of the set of feasible cache configurations.
\end{theorem}
%\begin{proof}
 %   The proof of the theorem is provided in Appendix \ref{app: Th2switch}
%\end{proof}
\begin{remark}
    From Theorems \ref{theorem:regret_unrestricted} and \ref{theorem:advswitch}, we conclude that Algorithm \ref{alg:FTPL} with unrestricted switching and input parameters $\mathbf{\eta}=(\eta_t=\alpha\sqrt{t})_{t\in \mathcal{T}}$ achieves $\mathcal{O}(\sqrt{T})$ adversarial regret by just using $\mathcal{O}(\sqrt{T})$ cache configuration switches.
\end{remark}
\subsubsection{Restricted Switching: } 
In this scenario, the cache content can only be changed in restricted time slots given by the set $\mathcal{T}$. Let $l_k \triangleq t_k-t_{k-1}$ define the time gap between the $(k-1)^{th}$ and $k^{th}$ switching slot, and $L \triangleq |\mathcal{T}|$ define the maximum number of allowed switches. By convention $t_0 = 1$ and $t_L = T$, we have $\sum_{k=1}^L l_k = T$.  The following theorem gives an upper bound on the adversarial regret of Algorithm \ref{alg:FTPL} under restricted switching with switching time slots given by the set $\mathcal{T}$.
 %is given by $l_k$, and thus the $k^{th}$ switching slot (wherein a switch may or may not occur) is given by $\sum_{i=1}^{k}l_i$. We also have $\sum_{i=1}^{L}l_i = T$. The policy (Algorithm \ref{alg:FTPL}) is used here whenever we have a switching slot. i.e., The cache placement step is done only during the switching slot, and the delivery step is performed in every slot.
\remove{\begin{theorem}\label{theorem:regret_restricted_switching}
Let $R_{(\eta, \text{UR})}^{A}(T)$ be the regret incurred by the policy (algorithm \ref{alg:FTPL}) in the adversarial unrestricted switching case with a horizon $T$. Then, the regret incurred by this policy in the restricted switching scenario with a learning rate $\alpha\sqrt{t}$ is upper-bounded as
\begin{equation}
R_{(\eta, \text{R})}^{A}(T) \leq R_{(\eta, \text{UR})}^{A}(T) +  \sum_{k=1}^{L}\frac{3r_{\max}^2(|\mathcal{S}|-1)l_k(l_k-1)}{4\alpha\sqrt{\pi}\sqrt{\sum_{i=1}^{k-1} l_i+1}} 
\end{equation}
Here $L$ is the number of switching slots until $T$.
\end{theorem}}
\begin{theorem}\label{theorem:regret_restricted_switching}
For an adversarial coded caching problem with $N$ files, $K$ users/caches, and cache size $MF$ bits, let $R_{(\eta, \text{R})}^{\mathcal{T}}(T)$ be the adversarial regret of Algorithm \ref{alg:FTPL} under restricted switching with switching slots $\mathcal{T}$ and input parameters $\mathbf{\eta}=(\eta_t=\alpha\sqrt{t})_{t\in \mathcal{T}}$. Then,
\begin{equation}
R_{(\eta, \text{R})}^{\mathcal{T}}(T) \leq R_{(\eta, \text{UR})}(T) +  \sum_{k=1}^{L}\frac{3r_{\max}^2(|\mathcal{S}|-1)l_k(l_k-1)}{4\alpha\sqrt{\pi}\sqrt{\sum_{i=1}^{k-1} l_i+1}}. \nonumber
\end{equation}
%Here $L$ is the number of switching slots until $T$.
\end{theorem}
%\begin{proof}
  %  The complete proof of this theorem is provided in Appendix \ref{app: resadv}.
%\end{proof}
%\begin{corollary}
 %   If $\mathcal{T}=[T]$, then $R_{(\eta, \text{R})}^{\mathcal{T}}(T) = R_{(\eta, \text{UR})}(T)$
%\end{corollary}

\begin{remark}
If $\mathcal{T}=[T]$, then we get back the unrestricted switching setting. In this case, the upper bound collapses to $R_{(\eta, \text{UR})}(T)$, and the second term in RHS becomes zero. Also, for a fixed intermittent switching period $l_k = l$ $\forall k$, i.e., we have $\left\lfloor\ T/l\right\rfloor +1$ total switching slots, and the second term in the upper bound is of order $\mathcal{O}(\sqrt{T})$. 
\end{remark}



